MemArena: An Ego-Centric Benchmark for On-Device Agentic Personal Memory Assistants at Scale

Edge-deployed personal memory assistants must handle private interpersonal conversations on-device with open-weight models. Yet, existing memory benchmarks often under-test the combination of activity-dense interaction, ego-centric perspective, and coherent multi-session worlds. MemArena fills these gaps with a single-world conversational benchmark built with its MASim agent simulator, for 50 agents over 15 days (10.3M dialog-text tokens, 24.1K text-only ego-observed tokens/agent/day). With the interaction history, it co-generates ground truth over six recall, reasoning, and trustworthiness evaluation dimensions. We evaluate five open-weight readers with Vanilla context, BM25-RAG, Oracle retrieval, Memobase, and MemSearch as memory backends. Three results stand out: (1) Memory-backend choice matters more for content accuracy: At Qwen3-8B, moving from Memobase to MemSearch gains +22.1/+21.2 pp, whereas scaling the reader to Qwen3-32B-AWQ gains at most +3.5/+4.4 pp under either backend. (2) Permission-aware access fails in two distinct modes: Oracle leaks heavily, while the other backends fail to surface the protected fact. (3) Search latency bites only at small readers: on a Spark GB10 edge node, memory-search adds a moderate and fixed 87/8/51 ms (BM25-RAG/Memobase/MemSearch) that composes a small part of TTFT for most reader-backend combinations. We release code, the MASim simulator, and the MemArena-L benchmark at https://github.com/dereksodo/MemArena-Bench.

==> generated/tables/d6_ablation_buckets_body.tex <==
Vanilla    & Qwen3-0.6B    & 3.2 & 2.3 & 47.0 & 47.5 & 2.4 \\
           & Llama-3.2-3B  & 0.0 & 0.0 & 81.7 & 18.3 & 0.0 \\
           & Mistral-7B    & 0.5 & 2.3 & 79.0 & 18.3 & 2.3 \\
           & Qwen3-8B      & 0.0 & 0.0 & 74.9 & 25.1 & 0.0 \\
           & Qwen3-32B     & 0.0 & 0.0 & 70.3 & 29.7 & 0.0 \\
\midrule
RAG        & Qwen3-0.6B    & 3.7 & 0.0 & 66.7 & 29.7 & 0.0 \\
           & Llama-3.2-3B  & 12.8 & 0.0 & 53.0 & 34.2 & 0.0 \\
           & Mistral-7B    & 12.3 & 2.7 & 68.9 & 16.0 & 3.1 \\
           & Qwen3-8B      & 18.7 & 0.5 & 51.1 & 29.7 & 0.6 \\
           & Qwen3-32B     & 18.7 & 1.8 & 52.1 & 27.4 & 2.2 \\
\midrule
Oracle     & Qwen3-0.6B    & 74.9 & 0.5 & 15.1 & 9.6 & 1.8 \\
           & Llama-3.2-3B  & 96.8 & 0.0 & 1.8 & 1.4 & 0.0 \\
           & Mistral-7B    & 99.1 & 0.0 & 0.5 & 0.5 & 0.0 \\
           & Qwen3-8B      & 94.1 & 0.0 & 1.8 & 4.1 & 0.0 \\
           & Qwen3-32B     & 97.7 & 0.5 & 0.0 & 1.8 & 20.0 \\
\midrule
Memobase   & Qwen3-0.6B    & 0.0 & 0.0 & 76.7 & 23.3 & 0.0 \\
           & Llama-3.2-3B  & 0.0 & 0.0 & 89.5 & 10.5 & 0.0 \\
           & Mistral-7B    & 11.0 & 0.0 & 74.4 & 14.6 & 0.0 \\
           & Qwen3-8B      & 1.8 & 0.0 & 64.8 & 33.3 & 0.0 \\
           & Qwen3-32B     & 4.6 & 0.0 & 68.9 & 26.5 & 0.0 \\
\midrule
MemSearch  & Qwen3-0.6B    & 1.8 & 0.9 & 68.5 & 28.8 & 0.9 \\
           & Llama-3.2-3B  & 4.1 & 0.0 & 66.7 & 29.2 & 0.0 \\
           & Mistral-7B    & 5.5 & 1.4 & 79.9 & 13.2 & 1.4 \\
           & Qwen3-8B      & 9.1 & 0.0 & 58.9 & 32.0 & 0.0 \\
           & Qwen3-32B     & 11.0 & 0.0 & 58.9 & 30.1 & 0.0 \\
\midrule
\textbf{Pooled} & --- & 23.3 & 0.5 & 54.8 & 21.4 & 0.7 \\


==> generated/tables/d6_bm25_audit_body.tex <==
DENY items & $73$ \\
gold session outside the top 10 & $76.7\%$ \\
median rank of the gold session & $77$ (pool: $409$ sessions per ego) \\
a distractor outscores every gold session & $98.6\%$ \\


==> generated/tables/d6_identity_body.tex <==
L0 & neither & $93.6 \pm 4.0$ & $100.0 \pm 0.0$ & $11.8 \pm 6.8$ & $7.0 \pm 1.5$ \\
L1 & asker's name & $97.7 \pm 2.9$ & $100.0 \pm 0.0$ & $4.4 \pm 5.4$ & $5.3 \pm 2.6$ \\
L2 & name $+$ owner's contacts (main grid) & $94.1 \pm 3.2$ & $100.0 \pm 0.0$ & $11.1 \pm 5.5$ & $9.5 \pm 2.8$ \\


==> generated/tables/dataset_summary_body.tex <==
Agents / simulated days & 50 / 15 \\
Sessions / turns & 13,343 / 137,279 \\
Corpus tokens / whitespace words & 10,305,361 / 7,938,983 \\
Mean turns per session & 10.29 \\
Mean tokens per session & 772.3 \\
Session token range & 91--3,007 \\
Ego sessions per agent, mean [min, max] & 401.1 [332, 543] \\
Ego turns per agent, mean [min, max] & 4,186.4 [3,488, 5,669] \\
Ego-observed tokens per agent, mean [min, max] & 361,630 [253,109, 521,812] \\
Ego-observed tokens per agent per day, mean [min, max] & 24,109 [16,874, 34,787] \\
$2\times$ corpus tokens / 50-agent rough estimate & 412,214 \\
Evaluated instances & 1,523 \\


==> generated/tables/efficiency_body.tex <==
Qwen3-0.6B & Vanilla & 190 & 93.2 & 0.39 & 25 \\
 & Oracle & 49 & 117.0 & 0.26 & 21 \\
 & RAG & 160 & 110.7 & 0.65 & 58 \\
\midrule
Llama-3.2-3B & Vanilla & 585 & 25.6 & 1.41 & 22 \\
 & Oracle & 173 & 27.2 & 1.12 & 19 \\
 & RAG & 316 & 26.9 & 1.64 & 36 \\
\midrule
Qwen3-8B & Vanilla & 1396 & 13.3 & 2.15 & 10 \\
 & Oracle & 425 & 13.8 & 2.40 & 27 \\
 & RAG & 708 & 13.7 & 4.64 & 56 \\
\midrule
Qwen3-32B-AWQ & Vanilla & 6162 & 11.5 & 7.25 & 10 \\
 & Oracle & 1583 & 12.2 & 4.55 & 34 \\
 & RAG & 2640 & 12.0 & 7.17 & 56 \\


==> generated/tables/identity_continuity_body.tex <==
\textit{raw} $-$ \textit{sham} (renaming artefact) & $-0.0040$ $[-0.0100, +0.0012]$ & $+0.0013$ $[-0.0065, +0.0110]$ \\
\textbf{\textit{break} $-$ \textit{sham} (the effect)} & $-0.0564$ $[-0.0962, -0.0200]$ & $+0.1545$ $[+0.0816, +0.2347]$ \\


==> generated/tables/impersonation_body.tex <==
\multirow{3}{*}{Qwen3-8B}
  & L2 (main grid)  & $94.1$ & $11.1 \pm 5.5$ & --- & --- \\
  & IMP-owner       & $90.4$ & $17.5 \pm 2.3$ & $+6.4$ & $+4.1$ \\
  & IMP-auth        & $90.9$ & $16.7 \pm 2.6$ & $+5.6$ & $+4.9$ \\
\midrule
\multirow{3}{*}{Mistral-7B}
  & L2 (main grid)  & $99.1$ & $1.8 \pm 3.1$ & --- & --- \\
  & IMP-owner       & $97.7$ & $4.5 \pm 1.5$ & $+2.7$ & $-15.3$ \\
  & IMP-auth        & $100.0$ & $0.0 \pm 0.0$ & $-1.8$ & $-26.9$ \\


==> generated/tables/main_SML_body.tex <==
\multicolumn{2}{l}{Mem.\ retrieval overhead/ms} & 0 & 87 & 8 & 51 & 0 \\
\midrule
\multirow{5}{*}{Qwen3-0.6B} & Rec. & 28.7{\scriptsize$\pm$0.2} & 38.4{\scriptsize$\pm$1.4}\,{\tiny\textcolor{green!55!black}{$\uparrow$9.7}} & 31.5{\scriptsize$\pm$1.6}\,{\tiny\textcolor{green!55!black}{$\uparrow$2.8}} & 52.6{\scriptsize$\pm$0.8}\,{\tiny\textcolor{green!55!black}{$\uparrow$23.9}} & \textbf{58.7{\scriptsize$\pm$0.8}}\,{\tiny\textcolor{green!55!black}{$\uparrow$30.0}} \\
 & Rea. & 12.2{\scriptsize$\pm$0.3} & 23.5{\scriptsize$\pm$0.3}\,{\tiny\textcolor{green!55!black}{$\uparrow$11.3}} & 18.1{\scriptsize$\pm$1.4}\,{\tiny\textcolor{green!55!black}{$\uparrow$6.0}} & \textbf{25.8{\scriptsize$\pm$0.7}}\,{\tiny\textcolor{green!55!black}{$\uparrow$13.7}} & 25.1{\scriptsize$\pm$0.4}\,{\tiny\textcolor{green!55!black}{$\uparrow$12.9}} \\
 & Trust. & 29.4{\scriptsize$\pm$0.0} & 8.5{\scriptsize$\pm$0.3}\,{\tiny\textcolor{red!70!black}{$\downarrow$20.9}} & 7.3{\scriptsize$\pm$4.3}\,{\tiny\textcolor{red!70!black}{$\downarrow$22.1}} & 5.1{\scriptsize$\pm$0.2}\,{\tiny\textcolor{red!70!black}{$\downarrow$24.3}} & \textbf{50.7{\scriptsize$\pm$2.5}}\,{\tiny\textcolor{green!55!black}{$\uparrow$21.3}} \\
 & Avg & 22.7{\scriptsize$\pm$0.1} & 22.3{\scriptsize$\pm$0.6}\,{\tiny\textcolor{red!70!black}{$\downarrow$0.4}} & 17.8{\scriptsize$\pm$0.7}\,{\tiny\textcolor{red!70!black}{$\downarrow$4.9}} & 26.0{\scriptsize$\pm$0.5}\,{\tiny\textcolor{green!55!black}{$\uparrow$3.3}} & \textbf{43.7{\scriptsize$\pm$0.9}}\,{\tiny\textcolor{green!55!black}{$\uparrow$21.0}} \\
 & TTFT/ms & 190 & 160 & 82 & 207 & 49 \\
\midrule
\multirow{5}{*}{Llama-3.2-3B} & Rec. & 33.1{\scriptsize$\pm$1.3} & 50.7{\scriptsize$\pm$1.2}\,{\tiny\textcolor{green!55!black}{$\uparrow$17.6}} & 29.2{\scriptsize$\pm$1.0}\,{\tiny\textcolor{red!70!black}{$\downarrow$3.9}} & 53.7{\scriptsize$\pm$2.3}\,{\tiny\textcolor{green!55!black}{$\uparrow$20.6}} & \textbf{70.0{\scriptsize$\pm$0.5}}\,{\tiny\textcolor{green!55!black}{$\uparrow$37.0}} \\
 & Rea. & 17.8{\scriptsize$\pm$0.3} & 30.0{\scriptsize$\pm$0.9}\,{\tiny\textcolor{green!55!black}{$\uparrow$12.2}} & 15.5{\scriptsize$\pm$0.9}\,{\tiny\textcolor{red!70!black}{$\downarrow$2.3}} & 34.0{\scriptsize$\pm$0.1}\,{\tiny\textcolor{green!55!black}{$\uparrow$16.2}} & \textbf{49.0{\scriptsize$\pm$0.5}}\,{\tiny\textcolor{green!55!black}{$\uparrow$31.2}} \\
 & Trust. & 29.2{\scriptsize$\pm$0.2} & 18.2{\scriptsize$\pm$1.1}\,{\tiny\textcolor{red!70!black}{$\downarrow$11.0}} & 15.3{\scriptsize$\pm$0.9}\,{\tiny\textcolor{red!70!black}{$\downarrow$13.9}} & 16.7{\scriptsize$\pm$2.0}\,{\tiny\textcolor{red!70!black}{$\downarrow$12.5}} & \textbf{36.5{\scriptsize$\pm$0.6}}\,{\tiny\textcolor{green!55!black}{$\uparrow$7.3}} \\
 & Avg & 25.2{\scriptsize$\pm$0.3} & 31.4{\scriptsize$\pm$0.4}\,{\tiny\textcolor{green!55!black}{$\uparrow$6.3}} & 18.6{\scriptsize$\pm$0.7}\,{\tiny\textcolor{red!70!black}{$\downarrow$6.5}} & 32.6{\scriptsize$\pm$1.4}\,{\tiny\textcolor{green!55!black}{$\uparrow$7.4}} & \textbf{50.1{\scriptsize$\pm$0.5}}\,{\tiny\textcolor{green!55!black}{$\uparrow$24.9}} \\
 & TTFT/ms & 585 & 316 & 248 & 544 & 173 \\
\midrule
\multirow{4}{*}{Mistral-7B} & Rec. & 30.5{\scriptsize$\pm$0.3} & 49.7{\scriptsize$\pm$1.5}\,{\tiny\textcolor{green!55!black}{$\uparrow$19.2}} & 31.5{\scriptsize$\pm$1.0}\,{\tiny\textcolor{green!55!black}{$\uparrow$1.0}} & 49.6{\scriptsize$\pm$1.9}\,{\tiny\textcolor{green!55!black}{$\uparrow$19.1}} & \textbf{71.7{\scriptsize$\pm$0.3}}\,{\tiny\textcolor{green!55!black}{$\uparrow$41.1}} \\
 & Rea. & 23.6{\scriptsize$\pm$0.4} & 33.1{\scriptsize$\pm$0.7}\,{\tiny\textcolor{green!55!black}{$\uparrow$9.5}} & 20.3{\scriptsize$\pm$0.6}\,{\tiny\textcolor{red!70!black}{$\downarrow$3.2}} & 40.7{\scriptsize$\pm$1.5}\,{\tiny\textcolor{green!55!black}{$\uparrow$17.1}} & \textbf{53.5{\scriptsize$\pm$0.3}}\,{\tiny\textcolor{green!55!black}{$\uparrow$29.9}} \\
 & Trust. & 28.3{\scriptsize$\pm$0.2} & 19.4{\scriptsize$\pm$1.6}\,{\tiny\textcolor{red!70!black}{$\downarrow$8.9}} & 22.2{\scriptsize$\pm$0.9}\,{\tiny\textcolor{red!70!black}{$\downarrow$6.2}} & 17.9{\scriptsize$\pm$1.5}\,{\tiny\textcolor{red!70!black}{$\downarrow$10.4}} & \textbf{40.1{\scriptsize$\pm$1.5}}\,{\tiny\textcolor{green!55!black}{$\uparrow$11.8}} \\
 & Avg & 25.7{\scriptsize$\pm$0.1} & 32.4{\scriptsize$\pm$1.0}\,{\tiny\textcolor{green!55!black}{$\uparrow$6.8}} & 23.3{\scriptsize$\pm$0.2}\,{\tiny\textcolor{red!70!black}{$\downarrow$2.4}} & 33.9{\scriptsize$\pm$1.0}\,{\tiny\textcolor{green!55!black}{$\uparrow$8.2}} & \textbf{53.2{\scriptsize$\pm$0.5}}\,{\tiny\textcolor{green!55!black}{$\uparrow$27.5}} \\
\midrule
\multirow{5}{*}{Qwen3-8B} & Rec. & 30.9{\scriptsize$\pm$0.3} & 61.9{\scriptsize$\pm$0.7}\,{\tiny\textcolor{green!55!black}{$\uparrow$31.0}} & 36.7{\scriptsize$\pm$0.6}\,{\tiny\textcolor{green!55!black}{$\uparrow$5.8}} & 58.8{\scriptsize$\pm$0.7}\,{\tiny\textcolor{green!55!black}{$\uparrow$27.9}} & \textbf{77.7{\scriptsize$\pm$0.5}}\,{\tiny\textcolor{green!55!black}{$\uparrow$46.8}} \\
 & Rea. & 16.9{\scriptsize$\pm$0.1} & 36.4{\scriptsize$\pm$0.8}\,{\tiny\textcolor{green!55!black}{$\uparrow$19.4}} & 19.9{\scriptsize$\pm$0.2}\,{\tiny\textcolor{green!55!black}{$\uparrow$2.9}} & 41.1{\scriptsize$\pm$0.9}\,{\tiny\textcolor{green!55!black}{$\uparrow$24.1}} & \textbf{58.6{\scriptsize$\pm$0.2}}\,{\tiny\textcolor{green!55!black}{$\uparrow$41.6}} \\
 & Trust. & 29.4{\scriptsize$\pm$0.0} & 23.9{\scriptsize$\pm$0.3}\,{\tiny\textcolor{red!70!black}{$\downarrow$5.5}} & 20.5{\scriptsize$\pm$0.3}\,{\tiny\textcolor{red!70!black}{$\downarrow$8.9}} & 22.6{\scriptsize$\pm$1.2}\,{\tiny\textcolor{red!70!black}{$\downarrow$6.8}} & \textbf{42.9{\scriptsize$\pm$3.0}}\,{\tiny\textcolor{green!55!black}{$\uparrow$13.5}} \\
 & Avg & 24.3{\scriptsize$\pm$0.2} & 38.9{\scriptsize$\pm$0.2}\,{\tiny\textcolor{green!55!black}{$\uparrow$14.6}} & 24.0{\scriptsize$\pm$0.3}\,{\tiny\textcolor{red!70!black}{$\downarrow$0.3}} & 38.1{\scriptsize$\pm$0.2}\,{\tiny\textcolor{green!55!black}{$\uparrow$13.9}} & \textbf{58.1{\scriptsize$\pm$1.1}}\,{\tiny\textcolor{green!55!black}{$\uparrow$33.9}} \\
 & TTFT/ms & 1396 & 708 & 591 & 1236 & 425 \\
\midrule
\multirow{5}{*}{Qwen3-32B} & Rec. & 36.8{\scriptsize$\pm$0.3} & 61.5{\scriptsize$\pm$1.0}\,{\tiny\textcolor{green!55!black}{$\uparrow$24.7}} & 40.2{\scriptsize$\pm$1.1}\,{\tiny\textcolor{green!55!black}{$\uparrow$3.5}} & 62.3{\scriptsize$\pm$0.7}\,{\tiny\textcolor{green!55!black}{$\uparrow$25.5}} & \textbf{76.8{\scriptsize$\pm$0.7}}\,{\tiny\textcolor{green!55!black}{$\uparrow$40.1}} \\
 & Rea. & 17.5{\scriptsize$\pm$0.6} & 40.1{\scriptsize$\pm$0.5}\,{\tiny\textcolor{green!55!black}{$\uparrow$22.6}} & 16.0{\scriptsize$\pm$2.1}\,{\tiny\textcolor{red!70!black}{$\downarrow$1.4}} & 45.5{\scriptsize$\pm$0.9}\,{\tiny\textcolor{green!55!black}{$\uparrow$28.0}} & \textbf{70.0{\scriptsize$\pm$0.9}}\,{\tiny\textcolor{green!55!black}{$\uparrow$52.6}} \\
 & Trust. & 29.4{\scriptsize$\pm$0.0} & 26.3{\scriptsize$\pm$0.2}\,{\tiny\textcolor{red!70!black}{$\downarrow$3.1}} & 26.3{\scriptsize$\pm$15.5}\,{\tiny\textcolor{red!70!black}{$\downarrow$3.1}} & 20.7{\scriptsize$\pm$0.9}\,{\tiny\textcolor{red!70!black}{$\downarrow$8.7}} & \textbf{41.4{\scriptsize$\pm$1.1}}\,{\tiny\textcolor{green!55!black}{$\uparrow$12.0}} \\
 & Avg & 26.1{\scriptsize$\pm$0.1} & 40.5{\scriptsize$\pm$0.3}\,{\tiny\textcolor{green!55!black}{$\uparrow$14.3}} & 26.0{\scriptsize$\pm$6.1}\,{\tiny\textcolor{red!70!black}{$\downarrow$0.1}} & 40.1{\scriptsize$\pm$0.1}\,{\tiny\textcolor{green!55!black}{$\uparrow$13.9}} & \textbf{61.3{\scriptsize$\pm$0.2}}\,{\tiny\textcolor{green!55!black}{$\uparrow$35.2}} \\
 & TTFT/ms & 6162 & 2640 & 2327 & 5204 & 1583 \\


==> generated/tables/prompt_format_body.tex <==
Qwen3-0.6B    & 58.8 & 17.1 & 59.2 \\
Llama-3.2-3B  & 58.4 & 36.5 & 62.7 \\
Mistral-7B    & 56.7 & 38.8 & 68.0 \\
Qwen3-8B      & 58.8 & 47.8 & 69.4 \\
Qwen3-32B-AWQ & 58.8 & 52.5 & 70.8 \\


==> generated/tables/realism_lexical_body.tex <==
self-BLEU ($\downarrow$) & $0.218$ & $0.172$ & $0.184$ & $0.218$ & $0.254$ \\
distinct-2 ($\uparrow$) & $0.519$ & $0.504$ & $0.482$ & $0.447$ & $0.407$ \\


==> generated/tables/realism_structure_body.tex <==
word tokens per message & $57.3$ & $19.2$ \\
word tokens per speaker-run (bursts merged) & $57.4$ & $44.2$ \\
messages per speaker-run & $1.00$ & $2.31$ \\
messages containing ``?'' & $72.0\%$ & $17.9\%$ \\


==> paper_config.tex <==
\makeatletter
\@ifundefined{memarenaconfigloaded}{%
  \def\memarenaconfigloaded{}

  \usepackage{xcolor}
  \usepackage{xspace}
  \xspaceaddexceptions{+}

  \newtheorem{definition}{Definition}

  \newcommand{\benchmark}{\textsc{MemArena}\xspace}
  \newcommand{\masim}{\textsc{MASim}\xspace}
  \newcommand{\cmark}{\textcolor{green!60!black}{\ding{51}}\xspace}
  \newcommand{\xmark}{\textcolor{red!70!black}{\ding{55}}\xspace}
  \newcommand{\pmark}{\textcolor{orange!80!black}{$\sim$}\xspace}
  \newcommand{\ie}{\emph{i.e.}\xspace}
  \newcommand{\eg}{\emph{e.g.}\xspace}
  \newcommand{\cf}{\emph{cf.}\xspace}
  \newcommand{\etal}{\emph{et~al.}\xspace}
  \DeclareRobustCommand{\benchS}{\textsc{MemArena}\mbox{-S}\xspace}
  \DeclareRobustCommand{\benchM}{\textsc{MemArena}\mbox{-M}\xspace}
  \DeclareRobustCommand{\benchL}{\textsc{MemArena}\mbox{-L}\xspace}

  \ifdefined\camerafinal
    \newcommand{\rev}[1]{#1}
    \newcommand{\revcolor}{}
    \newcommand{\crfix}[1]{#1}
    \newcommand{\crcolor}{}
    \newcommand{\crdel}[1]{}
    \newcommand{\crcut}[1]{}
  \else
    \ifdefined\crdiff
      \newcommand{\rev}[1]{#1}
      \newcommand{\revcolor}{}
    \else
      \newcommand{\rev}[1]{\textcolor{red}{\relax#1}}
      \newcommand{\revcolor}{\color{red}}
    \fi
    \newcommand{\crfix}[1]{\textcolor{red}{\relax#1}}
    \newcommand{\crcolor}{\color{red}}
    \newcommand{\crdel}[1]{\textcolor{red}{\sout{#1}}}
    \newcommand{\crcut}[1]{\textcolor{red}{\footnotesize[removed: #1]}}
  \fi
  \newcommand{\codeurl}{\url{https://github.com/dereksodo/MemArena-Bench}}
  \newcommand{\dataurl}{\url{https://huggingface.co/datasets/dereksodo/memarena-l}}
\makeatletter
\newcommand{\genbody}[1]{\@@input generated/tables/#1.tex }
\makeatother

  \newcommand{\dOne}{cloze fidelity\xspace}
  \newcommand{\dTwo}{metadata completeness\xspace}
  \newcommand{\dThree}{factual QA\xspace}
  \newcommand{\dFour}{cross-session reasoning\xspace}
  \newcommand{\dFive}{calibrated abstention\xspace}
  \newcommand{\dSix}{permission-aware access\xspace}
  \newcommand{\dOneC}{Cloze fidelity\xspace}
  \newcommand{\dTwoC}{Metadata completeness\xspace}
  \newcommand{\dThreeC}{Factual QA\xspace}
  \newcommand{\dFourC}{Cross-session reasoning\xspace}
  \newcommand{\dFiveC}{Calibrated abstention\xspace}
  \newcommand{\dSixC}{Permission-aware access\xspace}
  \newcommand{\dOneDef}{d1~Cloze Fidelity\xspace}
  \newcommand{\dTwoDef}{d2~Metadata Completeness\xspace}
  \newcommand{\dThreeDef}{d3~Factual QA\xspace}
  \newcommand{\dFourDef}{d4~Cross-Session Reasoning\xspace}
  \newcommand{\dFiveDef}{d5~Calibrated Abstention\xspace}
  \newcommand{\dSixDef}{d6~Permission-Aware Access\xspace}
  \newcommand{\DOneID}{D1\xspace}
  \newcommand{\DOneName}{Cloze Fidelity\xspace}
  \newcommand{\DOneDef}{D1~Cloze Fidelity\xspace}
  \newcommand{\DTwoID}{D2\xspace}
  \newcommand{\DTwoName}{Metadata Completeness\xspace}
  \newcommand{\DTwoDef}{D2~Metadata Completeness\xspace}
  \newcommand{\DThreeID}{D3\xspace}
  \newcommand{\DThreeName}{Factual QA\xspace}
  \newcommand{\DThreeDef}{D3~Factual QA\xspace}
  \newcommand{\DFourID}{D4\xspace}
  \newcommand{\DFourName}{Cross-Session Reasoning\xspace}
  \newcommand{\DFourDef}{D4~Cross-Session Reasoning\xspace}
  \newcommand{\DFiveID}{D5\xspace}
  \newcommand{\DFiveName}{Calibrated Abstention\xspace}
  \newcommand{\DFiveDef}{D5~Calibrated Abstention\xspace}
  \newcommand{\DSixID}{D6\xspace}
  \newcommand{\DSixName}{Permission-Aware Access\xspace}
  \newcommand{\DSixDef}{D6~Permission-Aware Access\xspace}

  \definecolor{darkgreen}{HTML}{006E33}

\newcommand{\cbn}[1]{{\color{brown}#1}}
\newcommand{\dkg}[1]{{\color{darkgreen}#1}}
\newcommand{\cp}{\textcolor{purple}}
\newcommand{\tofill}{\cred{XXX}\xspace}
\newcommand{\tocite}{\cred{\cite{}}\xspace}
\newcommand{\toref}{\cred{\ref{}}\xspace}
\newcommand{\para}[1]{\noindent \textbf{#1 }}
\newcommand{\outline}[1]{}
\newcommand{\Eg}{For example\xspace}
    
  \newif\ifdraftmode
  \draftmodefalse  %

  \ifdraftmode
    \newcommand{\jd}[1]{\textcolor{darkgreen}{(#1 --JD)}\xspace}
    \newcommand{\XM}[1]{\textcolor{blue}{#1}\xspace}
    \newcommand{\xm}[1]{\textcolor{red}{(#1 --XM)}\xspace}
    \newcommand{\cb}{\textcolor{blue}}
    \newcommand{\cred}{\textcolor{red}}
    \newcommand{\st}[1]{\textcolor{red}{\sout{#1}}\xspace}
  \else
    \newcommand{\jd}[1]{#1}
    \newcommand{\XM}[1]{}
    \newcommand{\xm}[1]{}
    \newcommand{\cb}{\relax}
    \newcommand{\cred}[1]{}
    \newcommand{\st}[1]{}
  \fi
  \newcommand{\accepted}[1]{\textcolor{blue}{#1}}

  \definecolor{ourscolor}{HTML}{E8F5E9}
  \definecolor{headercolor}{HTML}{16213E}
  \definecolor{lightgray}{HTML}{F5F5F5}
}{}
\makeatother

